Computation of Hadwiger Number and Related Contraction Problems: Tight Lower Bounds

We prove that the Hadwiger number of an $n$-vertex graph $G$ (the maximum size of a clique minor in $G$) cannot be computed in time $n^{o(n)}$, unless the Exponential Time Hypothesis (ETH) fails. This resolves a well-known open question in the area of exact exponential algorithms. The technique developed for resolving the Hadwiger number problem has a wider applicability. We use it to rule out the existence of $n^{o(n)}$-time algorithms (up to ETH) for a large class of computational problems concerning edge contractions in graphs.

==> conclusion.tex <==
%!tex root=mainClique.tex

\section{Conclusion}\label{sec:conclusion}

\hly{TODO: Note that the methods also extend to minor operations to classes of graphs.}



==> preamble.tex <==
\newcommand{\longversion}[1]{{#1}
\newcommand{\shortversion}[1]}

\usepackage{mathtools}
\usepackage[dvipsnames,svgnames,x11names]{xcolor}
\usepackage{amssymb,amsmath,mathrsfs}
\usepackage{soul}

\newcommand{\hlr}[1]{\sethlcolor{Salmon1}\hl{#1}\sethlcolor{yellow}} 
\newcommand{\hlg}[1]{\sethlcolor{PaleGreen2}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hlb}[1]{\sethlcolor{SkyBlue1}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hlo}[1]{\sethlcolor{Apricot}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hly}[1]{\sethlcolor{Gold}\hl{#1}\sethlcolor{yellow}}

\usepackage{listings}
\usepackage{mathrsfs}
%\usepackage[mathscr]{euscript}
\usepackage{amsfonts,amsthm,amsmath}
\usepackage{amstext}
\usepackage{graphicx,tikz}
\RequirePackage{fancyhdr}
\usepackage{boxedminipage}
\usepackage{todonotes}
%\usepackage[linesnumbered, boxed, algosection,noline]{algorithm2e}

\usepackage{graphics}
\usepackage{framed}
\usepackage{thm-restate}
\usepackage{thmtools}
\usepackage{enumerate}
\usepackage{float}
\usepackage{xspace}
%\usepackage{todonotes}

\newcommand{\OO}{\mathcal{O}}
\newcommand{\cO}{\mathcal{O}}

%\usepackage{vmargin}
%\setmarginsrb{1in}{1in}{1in}{1in}{0pt}{0pt}{0pt}{6mm}

\newcommand{\myparagraph}[1]{\smallskip\noindent{\textbf{\sffamily #1}}}

%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{lemma}{Lemma}[section]
%\newtheorem{claim}{Claim}[section]
%\newtheorem{corollary}{Corollary}[section]
%\newtheorem{definition}{Definition}[section]
%\newtheorem{observation}{Observation}[section]
%\newtheorem{proposition}{Proposition}[section]
%\newtheorem{redrule}{Reduction Rule}[section]
%\newtheorem{remark}{Remark}[section]
%\newtheorem{reduction}{Reduction Rule}[section]
%\newtheorem{conjecture}{Conjecture}[section]

\date{}
 
\newcommand{\defparproblem}[4]{
\vspace{1mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1  & {\bf{Parameter:}} #3 \\ \end{tabular*}
  {\bf{Input:}} #2  \\
  {\bf{Question:}} #4
  \end{minipage}
}\vspace{1mm}}

\newcommand{\defproblem}[3]{
\vspace{1mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1 \\ \end{tabular*}
  {\bf{Input:}} #2  \\
  {\bf{Question:}} #3
  \end{minipage}
}\vspace{1mm}}

%\usepackage{booktabs}
%\usepackage[pdftex, plainpages = false, pdfpagelabels, 
%                 %pdfpagelayout = useoutlines,
%                 bookmarks=false,
%                 bookmarksopen = true,
%                 bookmarksnumbered = true,
%                 breaklinks = true,
%                 linktocpage,
%                 pagebackref,
%                 colorlinks = true,  % was true
%                 linkcolor = blue,
%                 urlcolor  = blue,
%                 citecolor = red,
%                 anchorcolor = green,
%                 hyperindex = true,
%                 hyperfigures
%                 ]{hyperref}

% general
\newcommand{\yes}{\textsf{Yes}}
\newcommand{\no}{\textsf{No}}
\newcommand{\yesinstance}{\yes-instance}
\newcommand{\noinstance}{\no-instance}
\newcommand{\tw}{\mathtt{tw}}
\newcommand{\NP}{\textsf{NP}}
\newcommand{\coNP}{\textsf{co-NP}}
\newcommand{\FPT}{\textsf{FPT}}
\newcommand{\XP}{\text{XP}}
\newcommand{\WO}{\textsf{W[1]}}
\newcommand{\WOH}{\textsf{W[1]}-hard}
\newcommand{\WOC}{\textsf{W[1]}-complete}
\newcommand{\WTH}{\textsf{W[2]}-hard}
\newcommand{\WTC}{\textsf{W[2]}-complete}
\newcommand{\NPH}{\textsf{NP}-hard}
\newcommand{\NPC}{\textsf{NP}-complete}
\newcommand{\paraH}{\textsf{para-NP}-hard}
\newcommand{\ETH}{\textsf{ETH}}
\newcommand{\SETH}{\textsf{SETH}}
\newcommand{\nil}{\ensuremath{\mathtt{nil}}}
\newcommand{\cupdot}{\mathbin{\mathaccent\cdot\cup}}

% specific
\newcommand{\reduce}{\ensuremath{\mathtt{reduce}}}
\newcommand{\grid}{\ensuremath{\mathtt{Grid}}}
\newcommand{\conpart}{\ensuremath{\mathtt{ConPart}}}
\newcommand{\cost}{\ensuremath{\mathtt{cost}}}
\newcommand{\link}{\ensuremath{\mathtt{link}}}
\newcommand{\pf}{\ensuremath{\mathtt{pf}}}
\newcommand{\opt}{\ensuremath{\mathtt{opt}}}
\newcommand{\circulate}{\ensuremath{\mathtt{circulate}}}
\newcommand{\alg}{\ensuremath{\mathtt{Alg}}}

%%%%%%%%%%%%%%%%%%%
%% Problem names
%%%%%%%%%%%%%%%%%%%
 
\newcommand{\ProblemFormat}[1]{{\sc #1}}
\newcommand{\ProblemIndex}[1]{\index{problem!\ProblemFormat{#1}}}
\newcommand{\ProblemIndexBeg}[1]{\index{problem!\ProblemFormat{#1}|(}}
\newcommand{\ProblemIndexEnd}[1]{\index{problem!\ProblemFormat{#1}|)}}
\newcommand{\ProblemName}[1]{\ProblemFormat{#1}\ProblemIndex{#1}\xspace}
\newcommand{\ProblemNameX}[2]{\ProblemFormat{#1}\ProblemIndex{#2}\xspace}

\newcommand{\probVCS}{\ProblemName{$\eta$-Vertex Contraction Set}}
\newcommand{\probECS}{\ProblemName{$\eta$-Edge Contraction Set}}
\newcommand{\probrCDS}{\ProblemName{$r$-Connected Dominating Set}}
\newcommand{\probMaxLeafSptree}{\ProblemName{Max Leaf Spanning Tree}}
\newcommand{\probTWdel}{\ProblemName{Treewidth-$\eta$ Vertex Deletion}}
\newcommand{\probPWdel}{\ProblemName{Weighted Pathwidth-$\eta$ Vertex Deletion}}
\newcommand{\probTDepthdel}{\ProblemName{Weighted Treedepth-$\eta$ Vertex Deletion}}
\newcommand{\probFdel}{\ProblemName{Weighted Connected $\mathcal{F}$-Vertex Deletion}}
\newcommand{\probFdelc}{\ProblemName{Weighted Connected Planar $\mathcal{F}$-Vertex Deletion}}
\newcommand{\probFpack}{\ProblemName{$\mathcal{F}$-Packing}}
\newcommand{\probSdel}{\ProblemName{$\mathcal{S}$-Deletion}}
\newcommand{\probSpack}{\ProblemName{$\mathcal{S}$-Packing}}
% Commonly used names
\newcommand{\probVC}{\ProblemName{Vertex Cover}}
\newcommand{\probPlVC}{\ProblemName{Planar Vertex Cover}}
\newcommand{\probPVC}{\ProblemName{Partial Vertex Cover}}
\newcommand{\probPDS}{\ProblemName{Partial Dominating Set}}
\newcommand{\probPrDS}{\ProblemName{Partial $r$-Dominating Set}}
\newcommand{\probFVS}{\ProblemName{Feedback Vertex Set}}
\newcommand{\probIFVS}{\ProblemName{Independent Feedback Vertex Set}}
\newcommand{\probCycPacking}{\ProblemName{Cycle Packing}}
\newcommand{\probPlFVS}{\ProblemName{Planar Feedback Vertex Set}}
\newcommand{\probIS}{\ProblemName{Independent Set}}
\newcommand{\probWIS}{\ProblemName{Weighted Independent Set}}
\newcommand{\probMCIS}{\ProblemName{Multicolored Independent Set}}
\newcommand{\probDS}{\ProblemName{Dominating Set}}
\newcommand{\probrDS}{\ProblemName{$r$-Dominating Set}}
\newcommand{\probrSC}{\ProblemName{$r$-Scattered Set}}
%\newcommand{\probMDS}{\ProblemName{Minimum Dominating Set}}
\newcommand{\probPlDS}{\ProblemName{Planar Dominating Set}}
\newcommand{\probCDS}{\ProblemName{Connected Dominating Set}}
\newcommand{\probDST}{\ProblemName{Dominating Set on Tournaments}}
\newcommand{\probClique}{\ProblemName{Clique}}
\newcommand{\probMC}{\ProblemName{Multicolored Clique}}
\newcommand{\probPClique}{\ProblemName{Partitioned Clique}}
\newcommand{\probqSC}{\ProblemName{$q$-Set Cover}}
\newcommand{\probSC}{\ProblemName{Set Cover}}
\newcommand{\probDSP}{\ProblemName{Dominating Set with Pattern}}
\newcommand{\probOCT}{\ProblemName{Odd Cycle Transversal}}
\newcommand{\probEB}{\ProblemName{Edge Bipartization}}
\newcommand{\probHam}{\ProblemName{Hamiltonian Cycle}}
\newcommand{\probPlHam}{\ProblemName{Planar Hamiltonian Cycle}}
\newcommand{\probHamP}{\ProblemName{Hamiltonian Path}}
\newcommand{\probKPath}{\ProblemName{Longest Path}}
\newcommand{\probWKPath}{\ProblemName{Weighted Longest Path}}
\newcommand{\probthreeSAT}{\ProblemName{$3$-SAT}}
\newcommand{\probqSAT}{\ProblemName{$q$-SAT}}
\newcommand{\probcnfSAT}{\ProblemName{CNF-SAT}}
\newcommand{\probthreeCol}{\ProblemName{$3$-Coloring}}
\newcommand{\probqCol}{\ProblemName{$q$-Coloring}}
\newcommand{\probListColoring}{\ProblemName{List Coloring}}
\newcommand{\probOddSet}{\ProblemName{Odd Set}}
\newcommand{\probTuring}{\ProblemName{Short Turing Machine Acceptance}}
\newcommand{\probSI}{\ProblemName{Subgraph Isomorphism}}
\newcommand{\probGI}{\ProblemName{Graph Isomorphism}}
\newcommand{\probDFVS}{\ProblemName{Directed Feedback Vertex Set}}
\newcommand{\probDFAS}{\ProblemName{Directed Feedback Arc Set}}
%\newcommand{\probTw}{\ProblemName{Treewidth}} 
\newcommand{\probSteiner}{\ProblemName{Steiner Tree}}
\newcommand{\probSteinerF}{\ProblemName{Steiner Forest}} 
\newcommand{\probCVC}{\ProblemName{Connected Vertex Cover}}
\newcommand{\probCFVS}{\ProblemName{Connected Feedback Vertex Set}}
\newcommand{\OPT}{\operatorname{OPT}}
\newcommand{\probwTWcon}{\ProblemName{Weighted Treewidth-$\eta$ Vertex Contraction}}
\newcommand{\BMHitting}{\ProblemName{Boundaried Minor Hitting}}

